DT invariants from vertex algebras

We obtain a new interpretation of the cohomological Hall algebra $\mathcal{H}_Q$ of a symmetric quiver $Q$ in the context of the theory of vertex algebras. Namely, we show that the graded dual of $\mathcal{H}_Q$ is naturally identified with the underlying vector space of the principal free vertex algebra associated to the Euler form of $Q$. Properties of that vertex algebra are shown to account for the key results about $\mathcal{H}_Q$. In particular, it has a natural structure of a vertex bialgebra, leading to a new interpretation of the product of $\mathcal{H}_Q$. Moreover, it is isomorphic to the universal enveloping vertex algebra of a certain vertex Lie algebra, which leads to a new interpretation of Donaldson--Thomas invariants of $Q$ (and, in particular, re-proves their positivity). Finally, it is possible to use that vertex algebra to give a new interpretation of CoHA modules made of cohomologies of non-commutative Hilbert schemes.

==> commands.tex <==
\RequirePackage{amsmath,amssymb}%,amsthm}
\RequirePackage{etoolbox,bbm,xspace}
\RequirePackage{version,xparse}
%\RequirePackage[a4paper,margin=1.35in]{geometry}

%%%% Theorem environments
\ifx\notheorems\undefined
\theoremstyle{plain}
\newtheorem{theorem}{Theorem}[section]
\newtheorem*{itheorem}{Theorem}
\newtheorem{proposition}[theorem]{Proposition}
\newtheorem{lemma}[theorem]{Lemma}
\newtheorem{corollary}[theorem]{Corollary}
\newtheorem{claim}[theorem]{Claim}
\newtheorem{conjecture}[theorem]{Conjecture}
\theoremstyle{definition}
\newtheorem{remark}[theorem]{Remark}
\newtheorem{definition}[theorem]{Definition}
\newtheorem{example}[theorem]{Example}
\newtheorem{exercise}[theorem]{Exercise}
\theoremstyle{remark}
\newtheorem{rmr}[theorem]{Remark}
%\newtheorem{question}[theorem]{Question}
%\AtEndEnvironment{remark}{\hfill$\lozenge$}
%\AtEndEnvironment{example}{\hfill$\lozenge$}
\fi

%%%% Auxiliary commands
\def\mat#1{\ensuremath{#1}\xspace}
\def\dmat#1#2{\gdef#1{\mat{#2}}}
\def\csdmat#1#2{\csdef{#1}{\mat{#2}}}
\def\redef#1{\csletcs{t@#1}{#1}\csdmat{#1}{\csuse{t@#1}}}
\def\opr#1#2{\dmat#1{\operatorname{#2}}}
\def\opra#1#2{\csdmat{#1}{\operatorname{#2}}}
\def\oper#1{\csdmat{#1}{\operatorname{#1}}}
\def\DMO{\opr}
\makeatletter
\def\forlist#1#2{\@xp\forcsvlist\@xp{\@xp#1\@xp}\@xp{#2}}
% usage: \forlist\command\list
\makeatother

%%%% Operators. Usage: \GL
\forcsvlist\oper{
Vect,Mod,Rep,Ab,Grp,Com,Set,Top,Sch,Coh,Qcoh,Ob,Ring,Alg,
Map,Hom,End,Aut,Ext,Cat,Sh,Ind,RHom,Fun,Var,rad,
Ker,Im,deg,Tr,det,rk,diag,im,coker,tr,cone,add,
sk,cosk,colim,Res,Gal,Coker,dlog,
GL,SL,PGL,Gr,Lib,Conv,Sol,Tor,
Max,Spec,Ass,Ann,Quot,Pic,Sym,MHS,MHM,
td,ch,Supp,supp,vol,trdeg,lc,NS,Loc,Iso,per,gr,Der,Lie,
Log,Exp,Pow,ord,lcm,VB,Hilb,cl,SU,SO,Ad,ad,id}
\opr\Id{id}
\opr\lHom{\lb{Hom}}
\opr\lAut{\lb{Aut}}
\opr\lIso{\lb{Isom}}
\opr\hgt{ht}
\opr\chr{char}
\opr\udim{\mathbf{dim}}
\opr\cls{\mathsf{cl}}
\opr\mmod{mod}
\opr\Et{\mathsf{Et}}
\def\gl{\mathfrak{gl}}
\def\sl{\mathfrak{sl}}
\def\su{\mathfrak{su}}
\def\so{\mathfrak{so}}


%%%% Symbols
\def\mto{\mapsto}
\def\xto{\xrightarrow}
\def\lto{\leftarrow}
\def\xlto{\xleftarrow}
\def\emb{\hookrightarrow}
\def\lemb{\hookleftarrow}
\def\onto{\twoheadrightarrow}
\def\isoto{\xto{\,\smash{ 
	\raisebox{-3pt}{\ensuremath{\scriptstyle\sim}}
}\,}}
\dmat\es{\varnothing}%{\emptyset}
\def\bs{\backslash}
\def\sbs{\subset}
\def\sps{\supset}
\redef{iff}
\dmat\imp{\implies}
\dmat\xx{\times}
\dmat\dd{\partial}
\def\pd#1{\frac\dd{\dd#1}}
\def\iso{\simeq}
\def\ms{\backslash}
\def\bi{\mathbf i}
\def\bop{\bigoplus}
\def\ilim{\varprojlim} %inverse limit
\def\dlim{\varinjlim} %direct limit
\def\ts{\otimes}
\def\bts{\bigotimes}
\def\lb{\underline}
\def\ub{\overline}
\def\ubar#1{\mkern1.5mu\overline%
	{\mkern-1.5mu#1\mkern-1.5mu}\mkern1.5mu}
\def\oh{{\frac12}}
\dmat\Gm{\mathbb G_{\mathrm m}}
\dmat\one{\mathbbm1}
\def\qt{\delimiter"502F30E\mathopen{}} %/correct spacing
\def\dlim{\varinjlim} %direct limit
\def\ilim{\varprojlim} %inverse limit
\def\partof{\vdash}
\def\what{\widehat}
\def\tl{\tilde}
\def\wtl{\widetilde}
\def\inv{^{-1}}
\def\dual{^{\vee}}
\def\trp{^{\mathsf T}} %transpose
\dmat\pt{\mathbf{pt}}
\def\op{\mathrm{op}}
\def\st{\mathrm{s}}
\def\sst{\mathrm{ss}}
\def\nil{\mathsf {nil}}
\def\et{\mathrm{et}}
\def\ri{\mathrm i}
\def\sep{\mathrm{sep}}
\def\ab{\mathrm{ab}}
\def\top{\mathrm{top}}
\def\Ta{T^{\mathrm a}} %tensor algebra
\def\Tc{T^{\mathrm c}} %tensor coalgebra
\dmat\bul{\bullet}
\newdimen\bulh\settoheight\bulh{\bul}
\def\sbul{{\hspace{.5pt}\raisebox{.5\bulh}{%
	\scalebox{.5}{\raisebox{-.5\bulh}{\bul}}%
}}}%small bullet
\def\GIT{/\!\!/}
\def\qbinom{\genfrac{[}{]}{0pt}{}}
\def\ac{{\tiny\raisebox{2pt}{\textup{!`}}}}%anti-shriek
\newlength{\mylength}

\def\xmto#1{\,\tikz{
	\settowidth{\mylength}{\mat{#1}}
	\draw(0,1mm)--(0,-1mm);
	\draw[->](0,0)--(2\mylength,0)
	node[above,midway]{\mat{#1}};
	}\,}


%%%% Aphabets: \bA,\cA,\fA,\bfA,\sA
\def\defbb#1{\csdmat{b#1}{\mathbb{#1}}}
\def\defrm#1{\csdmat{r#1}{\mathrm{#1}}}
\def\defcal#1{\csdmat{c#1}{\mathcal{#1}}}
\def\deffrak#1{\csdmat{f#1}{\mathfrak{#1}}}
\def\defbf#1{\csdmat{bf#1}{\mathbf{#1}}}
\def\defsf#1{\csdmat{s#1}{\mathsf{#1}}}
\def\defall#1{\defrm{#1}\defbb{#1}\defcal{#1}\deffrak{#1}\defbf{#1}\defsf{#1}}
\forcsvlist\defall{A,B,C,D,E,F,G,H,I,J,K,L,M,N,O,P,Q,R,S,T,U,V,W,X,Y,Z}
\forcsvlist\deffrak{a,b,c,d,e,f,g,h,j,k,l,m,n,o,p,q,r,s,t,u,v,w,x,y,z}
\def\defbl#1{\csdmat{b#1}{\mathbf{#1}}} %lower case
\forcsvlist\defbl{a,b,c,d,e,g,h,i,j,k,l,n,o,p,q,r,s,t,u,v,w,x,y,z}
%\dmat\bk{\mathbbm k}
\dmat\bk{\Bbbk}

%%%% Greek letters
\dmat\al\alpha
%\dmat\be\beta
\dmat\ga\gamma
\dmat\de\delta
\dmat\la\lambda
\dmat\ta\tau
\dmat\hi\chi
\dmat\eps\varepsilon
\dmat\vi\phi
\dmat\te\theta
\dmat\ksi\xi
\dmat\si\sigma
\dmat\om\omega
\dmat\Ga\Gamma
\dmat\La\Lambda
\dmat\De\Delta
\dmat\Om\Omega
\dmat\Si{\Sigma}
\dmat\ze\zeta
\dmat\Te{\Theta}
\dmat\Na{\nabla}
\dmat\kp{\kappa}
\forcsvlist\redef{Phi,Psi,pi,mu,nu}

%%%% Structures
\def\set#1{\mat{\left\{#1\right\}}}
\def\sets#1#2{\left\{\left.#1\ \right\vert#2\right\}}
\def\ang#1{\mat{\left\langle#1\right\rangle}}
\def\angs#1#2{\ang{#1\rcol#2}}
\def\rbr#1{\left(#1\right)}
\def\sbr#1{\left[#1\right]}
\def\bra#1{\langle#1|}
\def\ket#1{|#1\rangle}
\def\n#1{\left\lvert#1\right\rvert}
%\def\nn#1{\left\lVert#1\right\rVert}
\def\eq#1{\begin{equation}#1\end{equation}}
\def\ov#1#2{{\substack{#1\\#2}}} % #1 over #2
\def\pser#1{[\![#1]\!]} %formal power series [[#1]]
\def\lser#1{(\;\!\!\!(#1)\!\!\!\;)} %formal Laurent series ((#1))
\def\pmat#1{\begin{pmatrix}#1\end{pmatrix}}
\def\vmat#1{\begin{vmatrix}#1\end{vmatrix}}
\def\smat#1{\left(\begin{smallmatrix}#1\end{smallmatrix}\right)}
\def\matr#1{\begin{matrix}#1\end{matrix}}
\def\pmatv#1#2{\left(\matr{#1}
	\hspace{.5ex}\middle|\hspace{.3ex}
	\matr{#2}\right)}
%\def\matr{\pmat}

%%%% Problems and solutions
%\newtheoremstyle{problem}{}{}{}{}\bf:{.5em}{}
%%%%\newtheoremstyle{problem}{}{}\em{}\bf:{.5em}{}
%\theoremstyle{problem}
%\newtheorem{prob}{Problem}
%\newif\ifsol
%\excludeversion{sol}
%\def\showsol{\soltrue%
%	\renewenvironment{sol}{\noindent{\bf Solution:}} {\hfill\qed}
%}

%%%% Diff
\def\br{\ \vspace{-.5ex}} %break after itemize
\def\dir#1#2{\noindent\textbf{(#1)$\implies$(#2).}}
\def\clm#1{\noindent\textbf{(#1)}\xspace} %claim, \cl should be used for classes
\def\lqq{\lq\lq}
\def\rqq{\rq\rq\xspace}
\def\qq#1{\lqq#1\rqq}
\def\tpdf{\texorpdfstring} %hyperref
\def\hl{\noindent\rule{\textwidth}{1pt}}

%%%% Words and phrases
\def\ie{i.e.\@\xspace} %id est
\def\cf{cf.\@\xspace} %confer
\def\eg{e.g.\@\xspace} %exempli gratia
%\def\fd{f.d.\@\xspace} % used for \mathfrak{d}
\def\etale{\'etale\xspace}
\def\qis{quism\xspace} %quasi-isomorphism
\def\wrt{with respect to\xspace}
\def\hint{\noindent\textbf{Hint:}\xspace}
\def\Wlog{Without loss of generality\xspace}
\def\tfae{the following are equivalent\xspace}
\def\nbd{neighborhood\xspace}

%%%% Citations
\def\defcite#1#2{%\defcite\moz{mozgovoy_DT}
	\DeclareDocumentCommand{#1}{o}
		{\IfValueTF{##1}{\cite[##1]{#2}}{\cite{#2}}\xspace}
}

%%%% Colons
\DeclareMathSymbol\col\mathrel{operators}{"3A}
\patchcmd\colon{:}{\col}{}{} %avoid the mention of :
{\catcode`:=\active 
\makeatletter\gdef:{\@ifnextchar={\col}\colon}}
\AtBeginDocument{\mathcode`:="8000}
\def\rcol{\col}

%\gdef:{\mskip2mu\mathchar"3A\mskip6mu}
% colon is \mskip2mu:\mskip6mu
\def\nop#1{\left.\col\hspace{-3pt}#1\hspace{-3pt}\col\right.}%normal order product

%%%% Indexed definition \idef{name}{optional name}
\DeclareDocumentCommand{\idef}{mo}{%
	\ifmmode#1\else\textit{#1}\fi%
	\IfValueTF{#2}{\index{#2}}{\index{#1}}%
}
%\def\itodo#1{\marginnote{\bf#1}}
%%\def\itodo{\todo[color=none,bordercolor=none]}
%\def\idef#1{\ifmmode\vadjust{\itodo{$#1$}}{#1}%
%\else\itodo{#1}\textbf{#1}\fi}

%%%% Table of contents style
%\makeatletter
%\renewcommand{\tocsubsection}[3]{%
%  \indentlabel{\@ifnotempty{#2}{
%  	\hspace*{1.1em}
%  	\makebox[2.3em][l]{\ignorespaces#1 #2.\hfill}
%	}}#3\dotfill}
%\makeatother


%%% Notes
\RequirePackage[framemethod=TikZ]{mdframed}

\newmdtheoremenv[backgroundcolor=green!15,roundcorner=5pt,innertopmargin=-2.5pt,linewidth=0]{innerNote}{Note}
%\newenvironment{notes}{\begin{innerNote}}{\end{innerNote}}

\newmdtheoremenv[backgroundcolor=yellow!15,
	innertopmargin=-2pt]{innerOld}{Old material}
\newenvironment{old}{\begin{innerOld}}{\end{innderOld}}

\newenvironment{comm}[1][brown!10]
{\begin{mdframed}[backgroundcolor=#1,linewidth=0]}
{\end{mdframed}}

\def\note#1{\comm#1\endcomm}

%\newtheorem{innerNote}{Note}
\newenvironment{notes}
	{\begin{mdframed}[backgroundcolor=green!15,
		roundcorner=5pt,innertopmargin=-2.5pt,linewidth=0]
		\innerNote
	}{\endinnerNote\end{mdframed}}

%\def\note#1{\par\noindent%
%	\colorbox{yellow!15}{\textbf{Note:} #1}}

%\RequirePackage{todonotes}
%\def\note#1{\
%	\todo[size=\normalsize,inline,bordercolor=yellow,
%	backgroundcolor=yellow!15]{#1}}

%\newenvironment{note}[1][yellow!15]
%{\begin{mdframed}[backgroundcolor=#1,linewidth=0]}
%{\end{mdframed}}

%\excludeversion{notes}
%\excludeversion{comm}
%\excludeversion{old}
%\def\note#1{}

%custom number side in equations, manual number: \tag{name}
\makeatletter
\def\leqnomode{\tagsleft@true\let\veqno\@@leqno}
\def\reqnomode{\tagsleft@false\let\veqno\@@eqno}
\makeatother

%%%%% Tikz commands
\newenvironment{ctikzcd}
	{\center\tikzcd}{\endtikzcd\endcenter}
\newenvironment{ctikz}
	{\center\tikzpicture}{\endtikzpicture\endcenter}
\tikzset{ % auxiliary styles
	crc1/.style={black,fill=yellow,radius=1cm},
	crc2/.style={black,fill=red,radius=1cm},
}

%custom theorem, can be used to list axioms (with labels)
\theoremstyle{plain}
\newtheorem{innercustomthm}{}
\newenvironment{customthm}[1]
  {\def\theinnercustomthm{#1}\innercustomthm}
  {\endinnercustomthm}

\DeclareDocumentCommand\sec{o}{
	\IfValueTF{#1}{\subsection{#1}}
			{\subsection{}\hspace{-1ex}}}

%%%%%%%%%%%%
\oper{wt}
\def\re{\mathrm{re}}
\def\im{\mathrm{im}}
\def\ser#1{\textcolor{red}{Sergey: #1}}
\def\st{\mathrm{st}}
%%%%%%%%%%%%

\def\f{\mathsf f}
\opr\NH{}
\def\be{\beta}
\def\M{\mathcal M}
\def\Q{\mathcal Q}
\def\P{\mathcal P}
\def\bd{\mathbf d}
\def\bw{\mathbf w}
\def\be{\mathbf e}
\def\e#1#2{\mat{e^{(#1)}_{#2}}}
\def\BM{\mathrm{BM}}
\def\coha{CoHA\xspace}
\def\cohas{\coha{s}\xspace}
\def\COHA{\coha}
\def\eprod#1{\,
	\tikz[baseline,anchor=base]
		{\node[draw,rectangle,inner sep=2pt]{$#1$};}\,}
\defcite\fren{frenkel_vertexa}
\def\io{\iota}
\oper{Ver}
\def\lEnd{\lb\End}
\def\oneb{\mathbf1}
\def\ws#1{\left\{#1\right\}}%weight shift
\def\fLm{\fL^\bw_\circ}
\oper{Coeff}
\def\frm{}
\def\fC{C}


